NADI 2021: The Second Nuanced Arabic Dialect Identification Shared Task

We present the findings and results of the Second Nuanced Arabic Dialect Identification Shared Task (NADI 2021). This Shared Task includes four subtasks: country-level Modern Standard Arabic (MSA) identification (Subtask 1.1), country-level dialect identification (Subtask 1.2), province-level MSA identification (Subtask 2.1), and province-level sub-dialect identification (Subtask 2.2). The shared task dataset covers a total of 100 provinces from 21 Arab countries, collected from the Twitter domain. A total of 53 teams from 23 countries registered to participate in the tasks, thus reflecting the interest of the community in this area. We received 16 submissions for Subtask 1.1 from five teams, 27 submissions for Subtask 1.2 from eight teams, 12 submissions for Subtask 2.1 from four teams, and 13 Submissions for subtask 2.2 from four teams.

==> eval.tex <==
\section{Evaluation}\label{sec:eval} 

Evaluation and task set up follow the MADAR 2019 shared task~\footnote{\url{https://sites.google.com/view/madar-shared-task/home}.}. The subtasks involved are as follows:
% \begin{itemize}
%   \item \textbf{Subtask 1:} Country-level dialect identification: A total of 30,957 tweets, covering 21 Arab countries. Distribution of the data is presented in Table~\ref{tab:country}. \mam{The dataset for both subtask 1 and subtask 2 can be accessed at \url{xxx}. More information about the data format can be found in the accompanying README file.} 
 
%   \item \textbf{Subtask 2:} is focused on state/province-level dialect identification. A total of 30,957 tweets, covering 100 states/provinces from all the 21 Arab countries. This is the same dataset as in Subtask 1, but with province labels. Class distribution of this dataset is described in Table~\ref{tab:state}. 
% \end{itemize}


Wet setup two codalabs for scoring participant systems. \footnote{The codalab for subtask I is accessible at: \url{https://competitions.codalab.org/competitions/24001?secret_key=66d8a9d9-3ac9-4ef2-bb74-6b8f3e287468}.}$^{,}$\footnote{Subtask II codalab is at: \url{https://competitions.codalab.org/competitions/24002?secret_key=53f14ab8-7db2-4011-9418-c95ee3b7ea2c}.} We keep the codalab for each task live post competition, for researchers who may have a desire to train models and score their systems on the shared task test set.

==> misc.tex <==
%Examples from the MSA-DA classifier, tagged as MSA:
%%%%%%%%%%%%%%%%%%%
\begin{enumerate}
\small
    \item <الحمد لله رب العالمين على نعمه التي لا تعد ولا تحصى ولم يغفل عن رزق كل خلقه.> 
    %<الحمد لله رب العالمين على نعمه التي لا تعد ولا تحصى ولم يغفل عن رزق كل خلقه وهو الرزاق \\ذو القوة المتين.>
    %\item <من أجل الجزائر من أجل البقاء و الازدهار ، من\\ المهم أن نكون قادرين على التكيف مع التغيير \\دون خيانة جذورنا التاريخية والثقافية و الدينية.>
    
    %\item <كيف سخر أمير قطر من دعوته لحضور قمة مكة؟>

    %\item <نحن شعب نعشق الخيال لأنه يأتي کما نحب .. تصبحون ع خير>

    % \item <البيض الفاسد يتدردب على بعضه يا صاحبي . قاتلهم الله>
    % \item <ما أبي اخذك منهم ، أبيك انت تبديني عليهم >
    \item <على بعضه يا صاحبي . قاتلهم الله> \colorbox{orange!15}{\<يتدردب>} <البيض الفاسد> 
    \item <عليهم> \colorbox{orange!15}{<تبديني>} <انت>  \colorbox{orange!15}{<أبيك>} <اخذك منهم ،>  \colorbox{orange!15}{<أبي>} <ما>     

\end{enumerate}


% Example 1 (softmax value=0.9951506853):

% <الحمد لله رب العالمين على نعمه التي لا تعد ولا تحصى ولم يغفل عن رزق كل خلقه وهو الرزاق ذو القوة المتين.>

% Example 2 (softmax value=0.9951434135):


% <من أجل الجزائر من أجل البقاء و الازدهار ، من المهم أن نكون قادرين على التكيف مع التغيير دون خيانة جذورنا التاريخية والثقافية و الدينية.>

% Example 2 (softmax value=0.9939758182):

% <كيف سخر أمير قطر من دعوته لحضور قمة مكة؟ URL via USER>

% Example xx (softmax value=0.993455708):


% <ومما أخبرني به صديقي 'مرزوق' أنه يقول: 'لن تنعم أي بلد من بلاد العرب بالحرية واستنشاق عبيرها، ما دامت الإمارات تعيش الهدوء داخل أراضيها.. يجب توجيه ضربات داخل الإمارات؛ حتى تنشغل بنفسها، بدلا من URL URL …>


% Example xx (softmax value=0.9887247682):


% <قوات الدفاع الجوي الملكي السعودي تعترض وتسقط طائرتين بدون طيار 'مسيرة' معادية أطلقتهما المليشيا الحوثية الإرهابية المدعومة من إيران باتجاه خميس مشيط . . شكرا رجال الدفاع الجوي>


% Example xx (softmax value=0.9219349027)
% <طهور ان شاء الله حبيبتي و الى اللقاء باذن الله تكوني احسن و افضل>

% Example xx (softmax value=0.915610373)

% <الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق الله يأخد الارق>


% Example xx (softmax value=0.9146798253)


% Example xx (softmax value=0.9146798253)

% <نحن شعب .. نعشق الخيال لأنه يأتي کما نحب .. تصبحون ع خير>

% Example xx (softmax value=0.7557364702)

% <ما أبي اخذك منهم ، أبيك انت تبديني عليهم .>


% Example xx (softmax value=0.7496300936)
% <البيض الفاسد يتدردب على بعضه يا صاحبي . قاتلهم الله .>

% Example xx (softmax value=0.7465314269)


% <هذا مثال صغير عن عقلية الشعب الجزايري الذي تسخن له الفرفارة بلخف و يصبح لا يفرق بين الحق و URL بين الواقع و الخيال يسمح بعاطفته التغلب على، URL يخرج الخراء من فمه.. الله يهدي ما خلق URL …>


% Example xx (softmax value=0.5319221616)


% <جماعة الإنتقالي لاخلوا لهم لاصاحب ولا رفيق خونوا الكل،، الله يملكنا العقول.>

% Example xx (softmax value=0.5001424551)

% <طشيتي اسرع من خبر عاجل الله وكيلج>




==> tables/baselines_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrr|rrrrrrrr}
\toprule
\textbf{}        & \multicolumn{8}{c}{{ \textbf{Country-level}}}                                                                                                                                                                                                                 & \multicolumn{8}{c|}{{ \textbf{Province-level}}}                                                                                                                                                                                                                \\ \cline{2-17}
\textbf{}        & \multicolumn{4}{c}{\textbf{Sub-task 1.1 (MSA)}}                                                                                               & \multicolumn{4}{c}{\textbf{Sub-task 1.2 (DA)}}                                                                                                & \multicolumn{4}{c}{\textbf{Sub-task 2.1 (MSA)}}                                                                                               & \multicolumn{4}{c}{\textbf{Sub-task 2.2 (DA)}}                                                                                                \\ \cline{2-17}
\textbf{}        & \multicolumn{2}{c}{\textbf{DEV}}                                     & \multicolumn{2}{c}{\textbf{TEST}}                                    & \multicolumn{2}{c}{\textbf{DEV}}                                     & \multicolumn{2}{c}{\textbf{TEST}}                                    & \multicolumn{2}{c}{\textbf{DEV}}                                     & \multicolumn{2}{c}{\textbf{TEST}}                                    & \multicolumn{2}{c}{\textbf{DEV}}                                     & \multicolumn{2}{c}{\textbf{TEST}}                                    \\ \cline{2-17}
\textbf{LM}      & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{$F_1$}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{$F_1$}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{$F_1$}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{$F_1$}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{$F_1$}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{$F_1$}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{$F_1$}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{$F_1$}} \\ \toprule
\textbf{mBERT}   & 24.48                           & 6.87                          & 24.30                           & 6.65                          & 32.94                           & 8.94                          & 32.70                           & 8.85                          & 1.50                            & 0.92                          & 1.80                            & 0.80                          & 2.88                            & 1.62                          & 2.56                            & 1.28                          \\ 
\textbf{XLM-R\textsubscript{B} }  & 23.66                           & 4.05                          & 22.38                           & 3.69                          & 29.86                           & 6.69                          & 28.90                           & 6.34                          & 1.80                            & 0.85                          & 1.54                            & 0.79                          & 2.46                            & 1.02                          & 2.48                            & 0.90                          \\ 
\textbf{XLM-R\textsubscript{L} } & 27.60                           & 10.87                         & 26.26                           & 10.15                         & 34.80                           & 12.03                         & 33.50                           & 11.07                         & 2.04                            & 1.17                          & 2.12                            & 1.45                          & 1.48                            & 0.66                          & 1.62                            & 0.61                          \\ 
\textbf{AraBERT} & 29.56                           & 13.31                         & 27.52                           & 12.27                         & 35.28                           & 12.04                         & 34.18                           & 11.28                         & 1.92                            & 1.13                          & 2.42                            & 1.21                          & 3.22                            & 1.90                          & 2.94                            & 1.46                          \\ 
\textbf{ARBERT}  & 33.30                           & \textbf{16.25}                         & 30.24                           & \textbf{14.47 }                        & 42.46                           & 20.70                         & 41.92                           & 20.61                         & 4.64                            & \textbf{3.73}                          & 4.62                            & \textbf{3.54}                          & 5.16                            & 3.60                          & 4.78                            & 3.07                          \\ 
\textbf{MARBERT} & 35.98                           & 15.36                         & 31.34                           & 12.20                         & 50.52                           & \textbf{27.13}                         & 49.22                           & \textbf{27.47 }                        & 4.26                            & 2.85                          & 4.60                            & 3.10                          & 7.36                            & \textbf{4.57}                          & 7.72                            & \textbf{4.60}                          \\ \toprule
\end{tabular}%
}
\label{tab:baselines}
\caption{\abdu{Results of baselines LMs over the $4$\textsuperscript{th} sub-tasks on DEV and TEST sets}}
\end{table*}

==> teams.tex <==
% \section{Teams}\label{sec:teams}
% We present teams here\dots 
